Multi-View Industrial Anomaly Detection with Epipolar Constrained Cross-View Fusion

Multi-camera systems provide richer contextual information for industrial anomaly detection. However, traditional methods process each view independently, disregarding the complementary information across viewpoints. Existing multi-view anomaly detection approaches typically employ data-driven cross-view attention for feature fusion but fail to leverage the unique geometric properties of multi-camera setups. In this work, we introduce an epipolar geometry-constrained attention module to guide cross-view fusion, ensuring more effective information aggregation. To further enhance the potential of cross-view attention, we propose a pretraining strategy inspired by memory bank-based anomaly detection. This approach encourages normal feature representations to form multiple local clusters and incorporate multi-view aware negative sample synthesis to regularize pretraining. We demonstrate that our epipolar guided multi-view anomaly detection framework outperforms existing methods on the state-of-the-art multi-view anomaly detection dataset.

==> backup/intro_bk.tex <==
\section{Introduction}
\label{sec:intro}


Detecting defects is essential to quality assurance in industrial processes. Due to the unconstrained presentation of defects, the task is often formulated as unsupervised anomaly detection. The research in industrial anomaly detection has been mainly supported by the introduction of diverse realistic datasets~\cite{bergmann2019mvtec,zou2022spot}. Most existing efforts into industrial anomaly detection still focus on detecting defects from a single snapshot of the object. In practice, industrial production line are often equipped with multiple cameras, capturing multi-view observations.  The new protocol is also referred to as multi-view industrial anomaly detection (MVIAD)~\cite{wang2024real}.

Despite the potential advantage of having multiple observations in MVIAD, existing approaches often do not fully exploit the related multi-view observations~\cite{wang2024real}. Directly applying the existing single-view methods often train a separate model on each viewpoint and inference is carried out independently. Ignoring the relationship among different views fails to fully unleash the advantage of multi-view information. In particular, the defect could be less discrminative in certain views, while being more pronounced from other viewpoints. Thus, fusing the information from multiple viewpoints may help better discern the anomalies on each view and eventually improving the decision of anomaly on the whole object. 

\begin{figure}[!h]
  \centering
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{ICCV_Multiview_Anomalydetection/sec/figure/epipolar_vis.png}
    \label{fig:short-a}
  \end{subfigure}
  \caption{Visualization of Epipolar Attention}
  \label{fig:vis_epi}
\end{figure}

Recent attempts to address multi-view anomaly detection focus on developing feature fusion techniques, feature alignment across different views, or self-supervised training~\cite{wang2022multiview}. These methods often consider multi-modality as multiple views which is not optimized for the multi-view camera system. Inspired by the success of attention based fusion~\cite{}, the Multi-View Adaptive Selection (MVAS) attention was proposed to tackle the multi-view fusion for MVIAD~\cite{he2024learning}. MVAS patchify feature maps and employs a typical cross-attention mechanism between different views to fuse the feature from different views. A reference patch is expected to aggregate features from the same location observed from other viewpoints and the selection of relevant patches in other viewpoints is determined by semantic similarity. The linear projection layers of the introduced cross-view attention module are learned by the reconstruction losses under the reverse distillation architecture~\cite{deng2022anomaly}. The success of MVAS suggests that correctly capturing the same patch across different views for feature fusion is beneficial to the overall prediction of anomaly.

Despite the success of existing multi-view anomaly detection approaches, we notice that these methods overlooked an important clue in the multi-view camera system. As seen from Fig.~\ref{fig:teaser}, a signifcant overlap between cameras exists in a typical multi-view defect inspection system, thus the observations of different camera views are constrained by the epipolar geomtry~\cite{hartley2003multiple}. More specifically, given a pixel $p_A$ in view A, we denote the the projection of the 3D point that induces pixel $p_A$ on view B as $p_B$. The homogeneous coordinates of $p_A$ and $p_B$ follow the epipolar constraint, $p_A^\top F p_B=0$ where $F$ is the fundamental matrix. This observation suggests that cross-view attention does not have to be solely based on semantic similarity~\cite{he2024learning} to identify the same patch across views but rather utilizing the epipolar geometry as guidance. To this end, we introduce an Epipolar Attention Module~(EAM) for cross-view fusion. For each patch in the reference view, we first identify possible corresponding patches in other support views following epipolar geometry. The corresponding patches should lie on the epipolar line. and then serve as the key and value. Cross-view attention then restricts the key and value to the patches that pass through epipolar line. 

As demonstrated in the experiments, the EAM will not be effective if the projection layers are randomly initialized. As opposed to the reverse distillation way of pretraining~\cite{deng2022anomaly}, memory bank based anomaly detection does not have an explicit training objective for learning the attention projection layers.  Therefore, we further propose a pre-training objective to optimize the projection layer weights. As a successful anomaly detection baseline, one-class classification minimizes the overall data volume in the feature space as a pretraining objective~\cite{ruff2018deep}. Noted the complex distribution of normal patterns in industrial image data, we propose a multi-center pretraining strategy by introduce multiple cluster centers and minimizes the data volume w.r.t. multiple centers. To prevent the model from degenerating to a trivial solution, i.e. mapping everything into a single or few targets, we further introduce synthesized negative samples as regularization. The negative samples are designed by considering the unique characteristics of epipolar attention. Finally, defects may present in non-deterministic ways in different viewpoints, thus maintaining a single memory bank for multi-view anomaly detection may not be the optimal way. To tackle this issue, we adopt a simple multi-view memory bank strategy by maintaining a view-specific memory bank for anomaly inference.

We conclude the contributions of this work as follows.

\begin{itemize}
    \item We are aware that defects are not equally visible and prominent in a multi-view camera system and existing methods employ purely data-driven approach for fusing features across camera views. We propose to exploit epipolar geometry as guidance for cross-view attention for more precise feature fusion.
    \item We build upon a memory bank based anomaly detection paradigm which does not have an explicit training objective. Thus we propose a multi-center pre-training strategy to optimize the parameters in the epipolar attention modules. Consistency based negative sample synthesis is also introduced to prevent trivial solutions.
    \item We demonstrate the effectiveness on the state-of-the-art multi-view industrial anomaly detection dataset without sacrificing the inference latency.
\end{itemize}


==> backup/method_bk.tex <==

\section{Methods}

%-------------------------------------------------------------------------
\subsection{Preliminaries of Industrial Anomaly Detection}
\begin{figure*}[h]
  \centering
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{ICCV_Multiview_Anomalydetection/sec/figure/ver2_0.png}
    \label{fig:short-a}
  \end{subfigure}
  \caption{Model pipeline graph******ver2.0}
  \label{fig:pipeline}
\end{figure*}
We first formally define the task of multi-view anomaly detection as follows. Each instance comes with images acquired from $V$ viewpoints, denoted as $x\in\mathbb{R}^{V\times 3\times H\times W}$. The task of multi-view anomaly detection is to make a prediction for each view and instance and identify the pixels belonging to the defects.

\noindent\textbf{Memory Bank based Anomaly Detection}: We revisit the memory bank based anomaly detection paradigm. Given a pre-trained encoder network $f(x;\Theta)$, e.g. ViT network, the network first patchify the input image into tokens and token features are learned via repeated transformer blocks. We take the tokenized feature for sample $x_i$, denoted as $z_{ij}\in\mathbb{R}^{H\cdot W/P^2\timesD}$, from the output of certain blocks of ViT encoder, where $D$, $H$, $W$ and $P$ refer to the feature channels, input image height, width and patch size, respectively. The memory bank $\mathcal{M}=\{m_k\}$ hosts the most representative tokenized features for anomaly prediction. Pushing all tokens from the normal training data into the memory bank is impractical due to the prohibitive data volume, therefore, core-set selection is often adopted to select a subset of tokens to store in $\mathcal{M}$~\cite{roth2022towards}. The anomaly score for each testing image is predicted at token level as Eq.~\ref{eq:pc_inf}. 

\begin{equation}\label{eq:pc_inf}
    s_{i}=\max_j\min_{m_k\in \mathcal{M}} ||z_{ij} - m_k||
\end{equation}

\noindent\textbf{Cross-View Attention for Multi-View Anomaly Detection}: Detecting anomalies with observations from multiple viewpoints is an emerging topic. The pilot study formulates the task as predicting anomalies from each view independently~\cite{wang2024real}. The vanilla practice overlooked a strong correlation between the information from different views. To further exploit the rich complementary information across multiple views, for each view, denoted as reference view, \cite{he2024learning} introduced a cross-view attention mechanism to aggregate information from other views, denoted as supporting views. Specifically, we redefine $z_i$ a tokenized/patchified feature map $z_i\in\mathbb{R}^{V\times H\cdot W/P^2\times D}$ encoded by the transformer network $f(x_i;\Theta)$, where $V$ refers to the number of views for a single instance. The attention between the $a$-th reference view $z_{ia}$ and supporting views $\{z_{ib}\}_{b\neq a}$ are simply formulated as the standard cross attention, where $W_Q$, $W_K$ , $W_V$ are learnable projection matrices.

\begin{equation}
\begin{split}
&Q=W_Qz_{ia}, K=W_Kz_{ib}, V=W_Vz_{ib},\\
    &Attn(z_{ia})=\frac{\text{softmax}(Q\cdot K)}{\sqrt{D}}
    \end{split}
    \end{equation}

Despite the improved performance from independent prediction, the cross-view attention is simply calcualted from semantic similarity of features. Learning the cross-view attention from a purely data-driven manner requires large amount of data and is prone to textureless and repetitive pattern images. In this work, we propose to exploit the epipolar geometry relationship to constrain the cross-view attention for better robustness and effeciency.

\subsection{Epipolar Attention for Multi-View Fusion}\label{sect:epiattn}

\noindent\textbf{Preliminaries of Epipolar Geometry}: In a non-degenerate stereo system, the pixel correspondence between two camera views are governed by the epipolar geometry. Given a pixel in view $a$, $p_a=[u_a,v_a,1]^\top$, the corresponding 2D project in view $b$, $p_b=[u_b,v_b,1]^\top$, lies on an epipolar line, subject to the epipolar constraint.

\begin{equation}
    p_a^\top F_{ab} p_b = 0
\end{equation}

The epipolar line in view $b$ is parameterized by $l_b=x_b^\top F_{ab}$. Given two views the fundamental matrix $F_{ab}$ can be efficiently estimated by 8-point algorithm~\cite{hartley2003multiple}. 




% Definition of Multi-view anomaly detection:
% In the context of multi-view anomaly detection , each sample $x \in \mathbb{R} ^{v \times C\times H\times W} $ consists of multiple views , where $v$ denotes the number of views. The model is tasked with estimating an instance-level anomaly score $S_{i} \in \mathbb{R^{v}}$ for each view and generating an anomaly map $S_{p} \in \mathbb{R} ^{ v \times C\times H\times W} $ that localizes defects within the view. Formally, the sample-level anomaly score $S_{x} \in \mathbb{R}$ is determined as: $S_{x} = \underset{S \in S_i}{max} \ S$
% Denote the feature representation of $z_{ij} \in \mathbb{R} ^{\frac{H*W}{p^{2}} \times p^{2} c}$ of sample $x_i$ with view $j$, extracted through an ViT-like encoder $f_{\theta}$ with patch size $p$. To facilitate cross-view information fusion, an aggregation function $\psi (z_{ij}, z_{ik})$ is employed to incorporate information from other views, and the feature employed for generating anomaly score and segmentation can be denoted as 
% \begin{equation}
% z_{ij} = \sum_{0\le k< v, k\ne j}\psi (z_{ij}, z_{ik}) \label{XX}
% \end{equation}

% Naïve approaches, such as direct feature concatenation or averaging, disrupt the original feature space and violate the independence among views. An alternative intuitive idea is to design a cross-view attention module for feature fusion. However, this approach introduces excessive visibility between different views. Specifically, it risks propagating anomalies detected in one view to another where they are not originally visible. Therefore, we employ an attention-based fusion module constrained by epipolar geometry, ensuring that feature interactions occur along corresponding epipolar lines. This enhances the alignment of features across views, leading to more robust anomaly detection. The details of this epipolar-constrained fusion model are elaborated in Section 3.2.

% In a two-view stereo system, the relationship between corresponding points in different camera perspectives is governed by epipolar geometry. Given a pixel in one view, its corresponding point in the second view must lie on a unique epipolar line, a fundamental constraint in stereo vision. let $x_{A}=(u,v,1)^{T}$ represent a pixel in view A in homogeneous coordinates. The corresponding epipolar line in view B is given by:
% \begin{equation}
% l_B = Fx_A \label{XX}
% \end{equation}
% where $F$ is the fundamental matrix, an essential $3×3$ matrix that encapsulates the geometric relationship between the two views. The equation of the epipolar line in view B follows the linear form:
% \begin{equation}
% au^{'} +bv^{'} +c=0 \label{XX}
% \end{equation}
% where denotes the pixel coordinates in view B, and $(a,b,c) $are the coefficients defining the epipolar line.




%-------------------------------------------------------------------------
% \subsection{Epipolar Attention for Multi-View Fusion}

\noindent\textbf{Cross-View Attention with Epipolar Constraint}: Contrary to the existing cross-view attention mechanism that solely relies upon the feature similarity, we propose to employ the epipolar geometry to provide as a guidance to the cross-view attention. %The introduced Epipolar Attention module~(EAM) exploits the epipolar geometry . 
Specifically, given a patch in reference view $z_{iaj}$, we first locate the center point of the patch $p_{iaj}$ following Eq.~\ref{eq:center_point}.

\begin{equation}\label{eq:center_point}
p_{iaj}=\begin{bmatrix} (\left \lfloor \frac{jP}{W}  \right \rfloor +0.5)\cdot P
 \\ (i \cdot\ mod{(\frac{W}{P})+0.5)\cdot P} 
 \\1
\end{bmatrix}
\end{equation}

Following the epipolar geometry, we know that the projection of point $p_{iaj}$ in the $b$-th supporting view lies on the epipolar line parameterized by $(p_{iaj}^\top F_{ab}) p_{ibk}=0$ where all $p_{ibk}$ satisfying the line equation could be the corresponding point. Therefore, we leverage this prior knowledge to constrain the cross-view attention. Since attention is applied at patch level, we first specify all possible patches by enumerating all patches in the supporting view that have an overlap with the epipolar line. The binary mask, $M_{ab}\in\{0,1\}^{H\cdot W/P^2\times H\cdot W/P^2}$, dictating the epipolar attention between view $a$ and $b$ can be obtained via Eq.~\ref{eq:epattn_mask} with $\delta$ indicating a threshold.

\begin{equation}\label{eq:epattn_mask}
\begin{split}
M_{ab}[j,k]&=\left\{\begin{matrix}1, \  \mathrm{if} \ d_{jk}\le \delta,
 \\0, \ \mathrm{otherwise}
\end{matrix}\right.\\
s.t.\quad d_{jk} &= \frac{| l_b p_{ibk} |}{\sqrt{(l_b)_1^2 + (l_b)_2^2}},\; l_b=p_{iaj}^\top F_{ab}
\end{split}
\end{equation}

The final Epipolar Attention Module~(EAM) thus writes in Eq.~\ref{eq:epattn}. %An illustration of the epipolar attention is shown in Fig.~\ref{fig:vis_epi}. 
This module replaces all cross-view attention modules in the backbone network to encourage feature aggregation across all supporting views.

\begin{equation}\label{eq:epattn}
    \begin{split}
        &z = W_O\sum Attn(z) V + z,\\
        s.t.\quad & Attn(z_{ia})=\frac{exp(Q_A^iK_B^j)}{ \sqrt{D}\sum_{k}^{} exp(Q_A^iK_B^k) M_{AB}(i,k) },\\
        &Q=W_Qz_{ia},\;K=W_Kz_{ib},\;V=W_Vz_{ib}
    \end{split}
\end{equation}


% To address the challenge of cross-view feature fusion, we propose an Epipolar Attention Module (EAM), which utilizes epipolar constraints to selectively aggregate information from corresponding regions in different views. Given a reference view $x_A \in \mathbb{R} ^{C\times H\times W}$ and a supporting view $x_B \in \mathbb{R} ^{C\times H\times W}$, a frozen feature encoder is implied to obtain the embedding $z_A$ and $z_B \in \mathbb{R} ^{\frac{H*W}{p^{2}} \times D}$, where D is the embedding dimension. In the attention module, extracted features are mapped to query $Q_A$, key $K_B$, and value $V_B$ representations using linear layer:
% \begin{equation}
% Q_A=W_Qz_A, \ K_B=W_Kz_B, \ V_B=W_Vz_B,  \label{XX}
% \end{equation}

% where $W_Q,W_K,W_V$ are learnable projection matrices. 
% Let $z_A^i$ denote the i-th patch in $z_A$, the corresponding pixel$p_A^i$ of $z_A^i$ can be obtained by:
% \begin{equation}
% p_A^i=\begin{bmatrix} (\left \lfloor \frac{ip}{W}  \right \rfloor +0.5)p
%  \\ (i \ mod{(\frac{W}{p})+0.5)p} )
%  \\1

% \end{bmatrix} \label{XX}
% \end{equation}
% where p is the patch size.

% Using Eq.xxxxx: we can obtain the corresponding epipolar line $l_B^i$ in view B. For every patch center $p_B^j$ in $z_B$, The per-patch distance of $p_B^j$ to $l_B^i$ can be calculated as:
% \begin{equation}
% d_{ij} =  \frac{\left | {l_{B}^{i}}^Tp_B^j \right | }{\sqrt{(l_{B}^{i})_x^2 + (l_{B}^{i})_y^2} }\label{XX}
% \end{equation}
% where $(l_{B}^{i})_x$ and $(l_{B}^{i})_y$ are the first two components of $l_{B}^{i}$. We then define a threshold $\delta $ to account for small misalignments or scale variations. The epipolar mask  is thus computed as:
% \begin{equation}
% M_{AB}(i,j)=\left\{\begin{matrix}1, \  \mathrm{if} \ d_{ij}\le \delta,
%  \\0, \ \mathrm{otherwise}

% \end{matrix}\right.\label{XX}
% \end{equation}
% As a result, $M_{AB} \in \left \{ 0,1 \right \} ^{(N,N)}$ enforces that patches from view A only attend to patches from view B lying on or near the epipolar line.
% The attention weights are computed as follows, incorporating the epipolar mask:
% \begin{equation}
% \alpha_{ij} = \frac{exp(Q_A^iK_B^j)}{ \sum_{k}^{} exp(Q_A^iK_B^k) M_{AB}(i,k) } \label{XX}
% \end{equation}
% The updated feature representation for each token in view A is then obtained by aggregating the values from view B:
% \begin{equation}
% \tilde{z} _{B}^{i} =\sum_{ j }^{} \alpha_{ij}V_B^j\label{XX}
% \end{equation}
% The final fused feature representation for view  is obtained via a linear transformation and residual connection:
% \begin{equation}
% \tilde{z}_A = W_O\tilde{z} _{B}+z_A\label{XX}
% \end{equation}
% where $W_O$ is a learnable transformation matrix




%-------------------------------------------------------------------------
\subsection{Multi-Center Pre-training}

In contrast to the epipolar transformer block where end-to-end training helps learn the linear projection layers~\cite{he2020epipolar}, memory bank based anomaly detection often does not have an explicit training objective to optimize the backbone network. Leaving these projection layers randomly initialized would compromise the overall performance. Therefore, we further propose a pre-training objective to help optimize the projection layers in EAM. Motivated by the success of unsupervised one-class classification, DeepSVDD~\cite{ruff2018deep} proposed a pre-training objective by reducing the total volume of a data-enclosing hypershpere in the feature space charaterzied by a radius $R>0$ and center $c\in\mathbb{R}^D$. However, optimizing towards a single feature cluster may not be feasible for modeling industrial objects of diverse appearance. As the inference strategy of PatchCore is by searching the nearest neighbor of a given testing sample in the memory bank, a good distribution of prototypes in the memory bank may follow a multi-modal distribution. This would translate into preserving multiple centers for pre-training.

For this purpose, we formulate a multi-center pre-training paradigm. First of all, we maintain $K$ cluster centers $\{c_k\in\mathbb{R}^D\}_{k=1\cdots K}$ in the patch feature space. The initialization of centers follow the K-Means clustering on all patch-level features. During the pre-training we iterate between assigning the patch to the closest prototype and minimizing the distance.

\begin{equation}
\begin{split}
    &\min_\Theta \frac{1}{N}\sum_{i,v,j} ||z_{ivj} - m_{k^*}||,\\
    s.t.\quad& {k^*}=\arg\min_{m_{k}\in\mathcal{M}} ||m_{k} - z_{ivj}||
\end{split}
\end{equation}

\noindent\textbf{Regularization with Synthesized Negative Sample}: Pretraining with clean patches alone may be easily prone to model collapse, i.e. encoding everything into a few identity features. To prevent the model from falling into trivial solutions, we further propose to regularize the pretraining with synthesized negative samples. Synthesizing negative samples in multi-view setup is more challenging than traditional single-view setups. Specifically, successful multi-view anomaly detection model should identify nuance defects from a reference view with the help from support views. This motivates us to explore a consistency based defect synthesis strategy.

Given a reference view $a$ and a support view $b$, we first select a patch in the support view, $p_{bk}$. We find all potential corresponding patches in the reference view as $\set{P}_a=\{p_{aj}\}$ following the epipolar geometry introduced in Sect.~\ref{sect:epiattn}. We extract the features for the patches in the reference view as $Z_a=\{z_{aj}\}\in$. Then, we mask out the patch in the support view and run forward inference again. This results in a new set of reference view features $\tilde{Z}_a=\{\tilde{z}_{aj}\}$. We compare the two set of features and choose the top $N_k$ patches as potentially anomalous patches in the reference view as negative patches $\set{Z}_{neg}$ as in Eq.~\ref{eq:neg_samp} where $\text{sortd}$ is in descending order. The same process is applied to each view. For each sample, we randomly sample one patch from one view to synthesize the anomaly. Each of the $V-1$ views are reference views, respectively, and the randomly selected view is the support view.

\begin{equation}\label{eq:neg_samp}
\begin{split}
    \tilde{\set{Z}}_{neg}&=\{\tilde{z}_{aj}\}_{j=1\cdots J^*[1:N_k]},\\
    s.t.\quad J^*&=\arg\text{sortd}_j||z_{aj}-\tilde{z}_{aj}||_2
\end{split}
\end{equation}

The negative patches are incorporated into pre-training by penalizing the logarithmic average distance to all cluster centers in the memory bank. Applying the logarithmic scaling will not overly encouraging the negative sample to stay from the prototypes. The loss for the $i$-th sample and $v$-th view writes as follows. 

\begin{equation}
    \mathcal{L}_{neg}(z_{i})=-\sum_{\tilde{z}_{ivj}\in\tilde{\set{Z}}_{neg}} \log\left(\frac{1}{|\set{M}_v|}\sum_{m_k\in\set{M}_v} ||\tilde{z}_{ivj}-m_k||_2\right)
\end{equation}



\noindent\textbf{Multi-View Memory Bank}: Existing memory bank based methods are mostly evaluated on single view dataset and a single memory bank is maintained to represent the distribution of normal samples. In the multi-view anomaly detection scenario, we notice that the significant viewpoint change could confuse the discrimination of good and defect patches. Therefore, we propose to maintain a separate memory bank for each individual view, giving rise to a multi-view memory bank $\{\set{M}_v\}_{v=1\cdots V}$. 

\noindent\textbf{Final Training Objective}: The final loss combining both positive and negative patches write in Eq.~\ref{eq:final_loss}.

\begin{equation}\label{eq:final_loss}
\begin{split}
 &\min_\Theta \sum_{i,v,j} ||z_{ivj} - m_{k^*}|| + \lambda\sum_{i}\mathcal{L}_{neg}(z_{i}),\\
    &s.t.\quad {k^*}=\arg\min_{m_{k}\in\mathcal{M}_v} ||m_{k} - z_{ivj}||
\end{split}
\end{equation}

% This motivates us to synthesize obvious defects in a support view B, e.g. by masking out certain patches $\mathcal{P}=\{p_bj\}$. For  we want to improve the model's capability to identify defects in the from  


% Inspired by the nearest neighbour searching mechanism of inference by PatchCore~\cite{roth2022towards}, we believe that a good distribution of prototypes in the 



% The introduced Epipolar Attention Module has multiple linear projection layers. 


% In order to train the parameters of the epipolar attention module while preserving the integrity of the pre-trained backbone , we adopt a patch-level multi-center pretraining strategy. Specifically, we freeze the backbone parameters and update the learnable weights in the epipolar attention block. Since our method relies on PatchCore-like inference, we aim to ensure that normal samples in the feature space remain tightly clustered at the patch level, thereby facilitating robust anomaly detection and segmentation. A straightforward approach, inspired by DeepSVDD, would be to minimize the volume of a data-enclosing hypersphere in output space $F$ that is characterized by radius $R > 0$ and center $c$. However, in a multiview setting with potentially diverse appearances for the same object, constraining all patch-level features from different views to a single center may degrade anomaly classification and segmentation performance. Instead, we employ multiple centers to accommodate the inherent heterogeneity of normal patterns across different views.
% Let $\tilde{z} _{A}^{i}$ denote the patch-level feature of the i-th patch from epipolar attention output in view A. We collect these features from all normal samples across all views and run the K-Means clustering algorithm on this collection of patch features to obtain $K$ cluster centers:
% \begin{equation}
% \left \{ c_1, c_2,\cdots , c_K \right \} , c_K \in \mathbb{R} ^d\label{XX}
% \end{equation}
% where $K$ is a hyperparameter. During pretraining, for each patch-level feature , we identify its closest center:
% \begin{equation}
% \phi (i)=arg \underset{1\le k \le K}{min} \left \| \tilde{z} _{A}^{i}-c_k \right \|_2\label{XX}
% \end{equation}
% We then pull $\tilde{z} _{A}^{i}$ toward $c_{\phi (i)}$ by minimizing the following loss:
% \begin{equation}
% \mathcal{L} = \frac{1}{N}\sum_{i=1}^{N} \left \| \tilde{z} _{A}^{i}-c_{\phi (i)} \right \| _2^2\label{XX}
% \end{equation}

% where $N$ is the total number of patch tokens in the training dataset. 
%-------------------------------------------------------------------------
\begin{figure*}[h]
  \centering
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{ICCV_Multiview_Anomalydetection/sec/figure/sample_vis.png}
    \label{fig:short-a}
  \end{subfigure}
  \caption{Anomaly segmentation results for two samples from the Real-IAD dataset: the audiojack class (left) and the USB class (right).}
  \label{fig:vis_sample}
\end{figure*}

\subsection{Inference}
During inference, we use the pretrained EAM and frozen backbone to obtain the patch memory bank $\mathcal{M} $ and perform coreset selection and anomaly scoring following PatchCore inference setting. We further refine each patch’s anomaly score using epipolar visibility from other views. Consider a test sample with multiple views . For a patch i in view A, we use the epipolar mask $M_{ij}(A,B)$ to locate all relevant patches j in view B. Denote the patch-level scores in view B by $s_B^j$. We compute the epipolar-refined score $\tilde{s} _A^i as$:
\begin{equation}
\tilde{s} _A^i=\alpha {s} _A^i+(1-\alpha)\frac{1}{\left | j|M_{ij}(A,B) \right | } \sum_{j}^{} M_{ij}(A,B){s} _B^j\label{XX}
\end{equation}

The overall sample-level anomaly score is then the maximum among all views:
\begin{equation}
s_{samp}=\underset{0\le i< v}{max} \ s_i\label{XX}
\end{equation}










